Geometry-Aware Learning of Maps for Camera Localization

Maps are a key component in image-based camera localization and visual SLAM systems: they are used to establish geometric constraints between images, correct drift in relative pose estimation, and relocalize cameras after lost tracking. The exact definitions of maps, however, are often application-specific and hand-crafted for different scenarios (e.g. 3D landmarks, lines, planes, bags of visual words). We propose to represent maps as a deep neural net called MapNet, which enables learning a data-driven map representation. Unlike prior work on learning maps, MapNet exploits cheap and ubiquitous sensory inputs like visual odometry and GPS in addition to images and fuses them together for camera localization. Geometric constraints expressed by these inputs, which have traditionally been used in bundle adjustment or pose-graph optimization, are formulated as loss terms in MapNet training and also used during inference. In addition to directly improving localization accuracy, this allows us to update the MapNet (i.e., maps) in a self-supervised manner using additional unlabeled video sequences from the scene. We also propose a novel parameterization for camera rotation which is better suited for deep-learning based camera pose regression. Experimental results on both the indoor 7-Scenes dataset and the outdoor Oxford RobotCar dataset show significant performance improvement over prior work. The MapNet project webpage is https://goo.gl/mRB3Au.

==> sec_results_pose.tex <==
\subsection{Pose Estimation Comparison }
\label{sec:result:comparison}
A big table to compare ours, ours with optimization and posenet~\cite{Kendall15iccv, Kendall17cvpr} and our implementation of posenet. 

==> sec_results_refining_sensor.tex <==
\subsection{Refining Noisy Sensor Inputs}
\label{sec:result:comparison:sensor}

\khnote{This is a section basically showing how our framework could refine the input sensors such as GPS data from the Robotcar datasets~\cite{RobotCarDatasetIJRR}}



==> sec_results_slam.tex <==
\subsection{Comparison to Sequential Pose Estimation}
\label{sec:result:comparison:slam}

\begin{figure}
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip=true,width=.99\linewidth]{ph}
\parbox[h]{.21\columnwidth}{\centering \scriptsize (a)}
\parbox[h]{.41\columnwidth}{\centering \scriptsize (b)}
\parbox[h]{.32\columnwidth}{\centering \scriptsize (c)}
\caption{Comparison to SLAM (ORB cite)...and the horizontal chart }
\label{fig:slam}
\vspace{-1em}
\end{figure}

==> supp_fig_robotcar.tex <==
\begin{figure*}
    \small
    \captionsetup[subfigure]{labelformat=empty}
    \centering
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/stereo_v2A_t.pdf}
        \vspace{-1.5em}
        \caption{\small Stereo VO (40.20m, 12.85\degree) }
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/posenet_t.pdf}
        \vspace{-1.5em}
        \caption{\small PoseNet (25.29m, 17.45\degree)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/vidvo_v2_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet (9.84m, 3.96\degree)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/gps_t.pdf}
        \vspace{-1.5em}
        \caption{\small GPS (7.03m, NA) }
    \end{subfigure}

    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/vidvo_online_1seq_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet+(1seq) (8.17m, 2.62\degree)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/vidvo_online_2seq_v2_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet+(2seq) (6.95m, 2.38\degree)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/vidvo_online_pgo_stereo_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet+PGO ({\bf 6.73m, 2.23\degree})}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/vidvo_online_gps_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet+(GPS) ({\bf 6.78m, 2.72\degree})}
    \end{subfigure}

    \vspace{1em}
    \line(1,0){300}
    \vspace{1em}

    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/stereo_v2AM_t.pdf}
        \vspace{-1.5em}
        \caption{\small Stereo VO (40.20m, 12.85\degree) }
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/posenetM_t.pdf}
        \vspace{-1.5em}
        \caption{\small PoseNet (26.23m, 19.75\degree)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/vidvo_v2M_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet (7.48m, 3.96\degree)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/gpsM_t.pdf}
        \vspace{-1.5em}
        \caption{\small GPS (6.54m, NA) }
    \end{subfigure}

    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/vidvo_online_1seqM_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet+(1seq) (6.46m, 2.62\degree)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/vidvo_online_2seq_v2M_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet+(2seq) ({\bf 5.64m}, 2.38\degree)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/vidvo_online_pgo_stereoM_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet+PGO (5.74m, {\bf 2.23\degree})}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar/vidvo_online_gpsM_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet+(GPS) ({\bf 4.95m, 2.72\degree})}
    \end{subfigure}
    \vspace{-.5em} 
    \caption{\small \textbf{Camera localization results on the LOOP scene (1120m long) of the
    Oxford RobotCar dataset~\cite{RobotCarDatasetIJRR}}. The ground truth camera trajectory
    is the black line, the star indicates the first frame, and the red lines show the
    camera pose predictions. The caption of each figure shows the mean translation error (m) and mean rotation error (\degree).
    MapNet+(1seq) uses one unlabeled sequence, while MapNet+(2seq) uses two unlabeled sequences.
    {\bf Left}: MapNet+ trained with unlabeled images and stereo VO. {\bf Right}: MapNet+ trained with unlabeled images and GPS data.}
    \label{fig:map_compare_robotcar}
\end{figure*}



==> supp_fig_robotcar_full.tex <==
\begin{figure*}
    \captionsetup[subfigure]{labelformat=empty}
    \centering
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar_full/stereoA_t.pdf}
        \vspace{-1.5em}
        \caption{\small Stereo VO (222.0m, 13.7\degree)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar_full/posenet_t.pdf}
        \vspace{-1.5em}
        \caption{\small PoseNet (125.6m, 27.1\degree)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar_full/vidvo_v2_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet (41.4m, 12.5\degree)}
    \end{subfigure}

    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures/robotcar_full/err_t_v2.pdf}
        \vspace{-.5em}
        \caption{\small Cumulative Distribution Translation Error}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar_full/vidvo_online_v2_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet+ (30.3m, 7.8\degree)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar_full/vidvo_online_pgo_stereo_v2_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet+PGO ({\bf 29.5m, 7.8\degree})}
    \end{subfigure}
    \hfill
    
    \vspace{1em}
    \line(1,0){300}
    \vspace{1em}

    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar_full/stereoAM_t.pdf}
        \vspace{-1.5em}
        \caption{\small Stereo VO (222.0m, 13.7\degree)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar_full/posenetM_t.pdf}
        \vspace{-1.5em}
        \caption{\small PoseNet (126.5m, 27.1\degree)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar_full/vidvo_v2M_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet (38.5m, 12.5\degree)}
    \end{subfigure}

    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar_full/err_t_v2M.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet+ (30.3m, 7.8\degree)}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar_full/vidvo_online_v2M_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet+ ({\bf 28.3m, 7.8\degree})}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/robotcar_full/vidvo_online_pgo_stereo_v2M_t.pdf}
        \vspace{-1.5em}
        \caption{\small MapNet+PGO (29.2m, {\bf 7.8\degree})}
    \end{subfigure}
    \hfill


    \vspace{-1em}
    \caption{\small Comparison of camera localization results on the FULL scene (9562m long) of the
    Oxford RobotCar dataset~\cite{RobotCarDatasetIJRR}. The ground truth camera trajectory
    is the black line, and the star indicates the first frame. The red lines show the
    results of stereo VO (provided by the dataset),
    our version of PoseNet+$\log\mathbf{q}$, MapNet, and its variations. The caption
    of each figure shows the mean translation error (m) and mean rotation error (\degree).
    A plot of the cumulative distribution of the translation error is also included.}
    \label{fig:map_compare_robotcar_full}
\end{figure*}


